Linked Adapters: Linking Past and Future to Present for Effective Continual Learning

Continual learning allows the system to learn and adapt to new tasks while retaining the knowledge acquired from previous tasks. However, deep learning models suffer from catastrophic forgetting of knowledge learned from earlier tasks while learning a new task. Moreover, retraining large models like transformers from scratch for every new task is costly. An effective approach to address continual learning is to use a large pre-trained model with task-specific adapters to adapt to the new tasks. Though this approach can mitigate catastrophic forgetting, they fail to transfer knowledge across tasks as each task is learning adapters separately. To address this, we propose a novel approach Linked Adapters that allows knowledge transfer through a weighted attention mechanism to other task-specific adapters. Linked adapters use a multi-layer perceptron (MLP) to model the attention weights, which overcomes the challenge of backward knowledge transfer in continual learning in addition to modeling the forward knowledge transfer. During inference, our proposed approach effectively leverages knowledge transfer through MLP-based attention weights across all the lateral task adapters. Through numerous experiments conducted on diverse image classification datasets, we effectively demonstrated the improvement in performance on the continual learning tasks using Linked Adapters.

==> sec/0_abstract.tex <==
\begin{abstract}
Continual learning refers to the ability of a system to learn and adapt to new tasks while retaining previously acquired knowledge. However, deep learning models suffer from catastrophic forgetting of knowledge learned from previous tasks while learning a new task. Moreover, retraining large models like transformers from scratch for every new task is costly. An effective approach to address continual learning is to use a large pre-trained model with task-specific adapters to adapt to the new tasks. Though this approach can mitigate catastrophic forgetting, they are not able to transfer knowledge across the tasks as each task is learning adapters separately. To address catastrophic forgetting and to enable knowledge transfer in continual learning, we propose a novel approach utilizing \textit{Linked Adapters} that incorporates a weighted attention mechanism to other task-specific adapters. Linked adapters use a multi-layer perceptron (MLP) to model the attention weights, which overcomes the challenge of backward knowledge transfer in continual learning. During testing, our proposed approach effectively leverages MLP-based attention weights across all the lateral task adapters, enabling knowledge transfer. Through numerous experiments conducted on diverse image classification datasets, our approach effectively demonstrated the improvement in continual learning through the successful transfer of knowledge in both forward and backward directions across the tasks.

\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}

In various applications, computational systems encounter the challenge of learning from a continuous stream of data and dynamically adjusting to their environment based on knowledge acquired from previous experiences. For example, an autonomous agent navigating the real world must be able to continually learn from a stream of data, ensuring that they retain knowledge gained from diverse and ever-shifting distributions without the threat of forgetting knowledge. Despite the remarkable performance of deep learning models in computer vision \cite{dosovitskiy2020image,krizhevsky2017imagenet}, they still struggle with the challenge of learning multiple tasks sequentially without forgetting previously acquired knowledge. The model's weights undergo significant alterations to accommodate the new task, often resulting in the forgetting of previously acquired knowledge. This phenomenon of forgetting knowledge acquired from previous tasks while attempting to learn new tasks, it is known as catastrophic forgetting \cite{mccloskey1989catastrophic}.  Achieving the capability to continuously learn from a continuous stream of tasks without compromising the retention of knowledge from prior tasks, all the while accommodating new tasks referred to continual learning \cite{parisi2018continual}. Continual learning approaches should be stable to learn new tasks without forgetting while also plastic to adapt new tasks is known as Plasticity-Stability dilemma~\cite{mermillod2013stability,grossberg2007consciousness}.


Vision transformers (ViTs) \cite{dosovitskiy2020image,carion2020end} have been established as a promising approach for solving computer vision tasks such as  classification, object detection and segmentation recently. However, Transformer-based models generally demand larger datasets and longer training times to achieve their full potential, primarily due to their extensive parameter count. 

To address this, various approaches \cite{dai2015semi,howard2018universal,radford2018improving}  proposed to use knowledge of  pre-trained large models (PLMs) like ViT \cite{dosovitskiy2020image} and DeiT \cite{deit} and fine-tune on new tasks. Finetuning on a new task will alter the weights of pre-trained network, and this is particularly problematic in continual learning scenarios where tasks are presented one after the other.  In such situations, we require a PLM that can adapt to new tasks without losing the knowledge gained from prior tasks along with limited parameter growth per task.

An effective approach to bringing continual learning capability in PLMs is through adapters~\cite{houlsby2019parameter,rebuffi2018efficient}. Adapters are small trainable parameters that are added to a pre-trained network to enable it to adapt to new tasks. To perform CL, pre-trained network is typically frozen, and only the task-specific adapter parameters are learned for each new task which allows it to retain information from prior tasks. Approaches like \cite{houlsby2019parameter} have shown the efficacy of adapters in fine-tuning on downstream tasks, showcasing their effectiveness in mitigating forgetting. The major limitation of the approach is not being able to transfer knowledge gained from one task to another because the model is frozen, and the task-specific parameters are learnt independently.


To deal with the aforementioned limitations, we propose a novel approach, \textit{Linked Adapters} that enables knowledge transfer across tasks in both forward and backward directions.\textit{Linked Adapters} have weighted attention-based lateral connections from other task-specific adapters to a particular task to enable knowledge transfer across the tasks. Specifically, these attention weights help to determine the degree of information flow from other tasks to the particular task. A major challenge here is to learn the attention weights in a CL setup, where we see tasks in a sequence. This makes it difficult to learn the attention weights from a later task to the current task. To address this challenge, we learn to predict the attention weights using a \textit{Multi-layer Perceptron (MLP)}. During the training phase, in addition to learning the adapter parameters, we learn the \textit{MLP} parameters which  generate the attention weights from previous to current task. During testing phase, the \textit{MLP} can be used to generate attention weights from subsequent tasks to any task which enable the backward transfer of knowledge in addition to the forward knowledge transfer without any extra effort in training.

The objective of employing \textit{MLP} based weighted attention is to ensure that knowledge can be transferred back to the initial tasks that might not have received sufficient knowledge from prior tasks. This bidirectional knowledge transfer mechanism helps in leveraging knowledge from subsequent tasks to benefit the initial tasks. Our experimental results demonstrate the effectiveness of the proposed \textit{MLP} based \textit{Linked Adapters} in transferring knowledge across the tasks on various image classification datasets.

Our main contributions are summarised as follows:
\begin{itemize} 
\item
We propose a novel approach \textit{Linked Adapters} that transfers the knowledge using weighted attention mechanism to other tasks.
\item We develop a \textit{MLP} based attention weight generation in \textit{Linked Adapters}  that enables backward transfer of knowledge to initial tasks without any extra training time.
\item We empirically show that \textit{Linked Adapters} able to transfer of knowledge across the tasks on  several image classification datasets in both forward and backward directions.
\end{itemize}




\section{Related Work}
Numerous efforts have been growing to deal with catastrophic forgetting in neural networks. Catastrophic forgetting limits neural networks in real-world scenarios where new data arrives continuously and the model must adapt to new tasks. Various proposed approaches in dealing forgetting can be broadly classified as Regularisation based approaches \cite{aljundi2018memory,kirkpatrick2017overcoming}, Replay based approaches~\cite{lopez2017gradient,shin2017continual,rebuffi2017icarl} and dynamic architecture based approaches \cite{yoon2017lifelong,rusu2016progressive}. Regularisation based approaches like Elastic weighted Consolidation (EWC) \cite{kirkpatrick2017overcoming}, imposes constraints on the important parameters of the old tasks while also allowing other parameters to adapt to new tasks. Another similar approach Synaptic Intelligence (SI) \cite{zenke2017continual}, that assigns importance score to each neuron based on its contribution to the performance on previous tasks.

Rehearsal or replay based approaches replays the stored or synthetic samples of previous tasks while learning new tasks to mitigate forgetting. During training, model is trained on samples of previous tasks along with new task data.  Synthetic samples can be generated using Variational Auto Encoders (VAEs) or Generative Adversarial networks (GANs). Various approaches like Deep Generative reply (DGR) \cite{shin2017continual}, Gradient Episodic Memory (GEM) \cite{lopez2017gradient}, iCaRL \cite{rebuffi2017icarl} have been proposed based on this strategy. Major limitation with replay-based approach is with buffer size as the number of tasks grows number of samples stored per task will become less and it leads to forgetting of previous tasks. Dynamic architecture-based approaches grow the entire or specific part of the network to accommodate new tasks. Progressive Neural Networks (PNNs) \cite{rusu2016progressive} are the one of the earliest works to expand entire network for each task and maintain lateral connections from old network. DEN \cite{yoon2017lifelong} grows only limited units of the network and identifies neurons that are important to selectively trains them for current task. Dynamic neural network can accommodate new tasks at the cost of growing the parameters.

Transformers based models are traditionally built for NLP tasks however are now commonly applied to range of vision tasks. ViT \cite{dosovitskiy2020image} is the one of the earliest transformer-based architecture that splits the images into multiple smaller patches are given as input to transformer. With larger number of parameters in transformer compared to other models, to get full potential it need to be trained on larger datasets. In practice, data not often larger every time, to deal with such cases we need to use the knowledge of pre-trained model while learning downstream tasks. 
Various approaches \cite{dai2015semi,howard2018universal,radford2018improving}, demonstrated the impact of pre-trained models in transfer learning. A Transformer model BERT \cite{bert} trained with large text corpus data has shown state-of-the-art results in many NLP tasks while pre-trained DeiT \cite{deit} and ViT \cite{dosovitskiy2020image} able to improve the performance on Cifar~\cite{cifar100}, ImageNet~\cite{imagenet}  and several classification tasks. Usually, pre-trained models are fine-tuned for specific downstream tasks to leverage their existing knowledge. However, in a continual learning scenario where tasks are sequentially presented, updating the entire network for each new task can be undesirable as it leads to the loss of initial pre-trained information.

Various approaches~\cite{houlsby2019parameter,rebuffi2018efficient} have been proposed to update few task specific parameters for each downstream task instead of finetuning on all the parameters. Residual adapters~\cite{rebuffi2018efficient} are one of the earliest works in adapters that add learnable residual layers for pre-trained ResNet for transfer learning in multi domain learning. These learnable residual layers are architecture specific can't be generalised to transformer-based models. 
Recently, transformer specific adapters are proposed for learning many downstream tasks in NLP and shown finetuning downstream tasks on pre-trained models is parameter inefficient as it updates the weighs of whole network and proposed to update only few tasks specific parameters using Adapters~\cite{houlsby2019parameter}. ADA~\cite{ermis2022continual} maintains a pool of adapters whenever new task comes an adapter from pool is selected and distill it along with new adapter. As the number of tasks grows, each adapter has to accommodate multiple tasks might lead to forgetting as adapter itself has very few parameters.



\section{Background}
\subsection{Problem Formulation}

Continual learning assumes tasks to arrive in a sequential manner, and there exists a limited memory so we cannot store the previous task data or model parameters. Our goal is to effectively learn a set of \(m\) image classification tasks, denoted as \( \mathcal{T}=\{\mathcal{T}^{1},\mathcal{T}^{2},\ldots,\mathcal{T}^{m}\} \), as they arrive in sequence. Each task \(t\in\mathcal{T}\) is associated with data  \((X^{t}, Y^{t})\), where \(X^{t}=\{x_{i}^{t}\}_{i=1}^{N^t}\) represents the input data points with $x_{i}^{t} \in \mathcal{X}$, and \(Y^{t}=\{y_{i}^{t}\}_{i=1}^{N^t}\) represents the corresponding output data points with $y_{i}^{t} \in \mathcal{Y}^t$. \(N^t\) represents the number of samples in task $t$ and let $\mathcal{Y} = \{\mathcal{Y}^1, \ldots, \mathcal{Y}^m \}$ represents the collection of classes across all the tasks. Our objective is to learn a model $f{(\cdot, {\Theta}}):\mathcal{X}\to\mathcal{Y}$ with parameter $\Theta$ that can provide a good generalization performance across all the tasks.

\subsection{Adapters}

Training large models like transformers from scratch on new tasks is time consuming and typically needs larger datasets to train. An efficient way is to use pre-trained models trained on larger datasets. Finetuning pre-trained models on downstream tasks will be able to transfer knowledge and often helps in faster convergence. Finetuning updates the weights of entire pre-trained network which is not desirable. Log likelihood objective function for finetuning on downstream task $t$ where output variable $y^t$ given input $x^t$ and pre-trained model weights $\Theta$ can be defined as
\begin{align*}
    \max_{\Theta,\Psi^t} \sum_{i=1}^{N^t} {  \log {\mathcal{P}(y^t_i| x^t_i,\Theta,\Psi^t)}}
\end{align*}
where $\Psi^t$ is parameters of task specific output classifier head, The classifier head is a simple feed forward layer that maps the pre-trained model's hidden representations to the output space $\mathcal{Y}^t$. 
 
 In continual leaning scenario, task arrives in sequential manner, finetuning parameters on every new task loses information of pre-trained data. Adapters \cite{houlsby2019parameter} can solve limitations of finetuning on downstream tasks without updating pre-trained weights $\Theta$ by adding task specific parameters for each task. Typically, structure of an adapter $(\mathcal{A}^{t})$ involves a bottleneck architecture with $MLP$ layers that can downsample $(D^{t})$   and then upsample $(U^{t})$  the representations. To learn downstream task $t$, Adapters are added at every layer of transformer $i.e.,$ $\tilde{h}^{t}_{k}=U_{k}^t (D_{k}^{t}(\bar{h}^{t}_{k}))$ where $\bar{h}^{t}_{k}$ is hidden representation input to adapter, $\tilde{h}^{t}_{k}$ is hidden representation output of adapter at $k^{th}$ layer . Only few task specific adapter parameters($\Phi^t$) are learnt for each task by keeping pre-trained parameters $\Theta$ frozen. The objective function is to maximize the log-likelihood of $y^t$ given the input $x^t$, task specific adapter parameters $\Phi^t$ across sequence of tasks in continual learning setup. Learning in current task $t\in\mathcal{T}$ can be defined as:

\begin{align*}
  \max_{\Phi^{t},\Psi^t} \sum_{i=1}^{N^t}  { \log {\mathcal{P}(y^t_i|x^t_i,\Theta^\dagger,\Phi^t,\Psi^t)}}
\end{align*}

 % Adapters are added at every layer of transformer denoted as \(U_{t}=\{U^{k}_{t}\}_{k=1}^{l}\), \(D_{t}=\{D^{k}_{t}\}_{k=1}^{l}\) where $l$ denotes number of layers in transformer.



% \begin{equation}
%     \max_{\Phi^{t}} \sum_{x,y\in t} {  \log {\mathcal{P}(y^t/x^t,\Theta_p^f,\Phi^t)}}
% \end{equation}



Here, $\Theta^\dagger$ is pre-trained model weights where $\dagger$ indicates weights are frozen, and the task specific adapter parameters $\Phi^{t}$ are learnt for each task independently. The goal of the adapter training is to learn $\Phi^t$ that maximize this log-likelihood on the training set. As pre-trained model weights are frozen, learning separate adapters independently won't transfer knowledge across tasks. In continual learning scenario, we need a model that transfers knowledge across the tasks.


\begin{figure*}
  \centering

    \includegraphics[width=\linewidth]{sec/architecture (9).png}
     \caption{Figure \ref{fig:architecture}.a. demonstrates \textit{Linked Adapters} during training where lateral connections from previous tasks are connected to current task $t$ to enable knowledge transfer and their corresponding attention weights are being generated by \textit{MLP} . Figure \ref{fig:architecture}.b. demonstrates \textit{Linked Adapters} during testing where lateral connection from previous tasks and subsequent tasks are added to to current tast $t$ enable knowledge transfer from both directions where \textit{MLP} generates attention weights of subsequent tasks without any extra training.}
     \label{fig:architecture}
\end{figure*}






\section{Linked Adapters}
In a continual learning scenario where tasks are learned sequentially, if tasks share common underlying representations, knowledge gained from one task can be leveraged to facilitate learning in subsequent tasks. However, a significant limitation arises when employing separate and independent adapters \cite{houlsby2019parameter}, as this approach involves freezing the pre-trained model and restricting learning to task-specific parameters in isolation. To address this limitation, we aim to propose \textit{Linked Adapters}, that can transfer knowledge across tasks. In \textit{Linked Adapters}, each adapter has a systematic lateral connections to the adapters from all other tasks to enable knowledge transfer across tasks. The challenge arises from the uncertainty of determining the degree of information flow required, as information should ideally flow more prominently between similar tasks and with lesser emphasis on dissimilar tasks. To address this challenge, a more sophisticated mechanism, such as the utilization of attention weights, becomes necessary to control the flow of information in a manner tailored to each task.   However, in a CL scenario where tasks arrive sequentially, learning the attention weights becomes even more challenging as we don't see all the tasks and their corresponding adapters together. To address this, we employ a \textit{Multi-Layer Perceptron (MLP)} that is trained to generate the attention weights. During training, \textit{MLP} learns to generate the attention weights for the lateral connections from the previous task adapters. Through the attention weights, the current task model learns which information to keep from previous tasks. During testing, this \textit{MLP} proves invaluable for leveraging the knowledge gained from subsequent tasks by predicting the attention weights to the subsequent tasks. This benefits the initial tasks that receive limited information otherwise from the tasks prior to them. We achieve this knowledge transfer across the tasks without requiring any additional training to learn the attention weights from later tasks. In the following sections, we will discuss in detail about working of \textit{Linked Adapters}.


\subsection{Linked Adapter Training }
During training, we see the tasks in a sequence, \textit{Linked Adapters} maintains lateral connections, which establish links between the representations of previous task adapters to the current learning adapter as in Figure~\ref{fig:architecture}.a. A \textit{MLP} $f_{h}(.,\Theta_{h})$ is learnt along with task-specific adapter parameters to generate forward attention weights between every previous task to current task. In order to generate forward attention weights $\beta^{pt}$ between previous task $(p)$ adapter representation to current task $t$, \textit{MLP} takes task specific embeddings of previous task $\mathbf{e}^p$ and task embedding of current task $\mathbf{e}^t$ as input. The generation can be defined as  
\begin{equation}\label{eq:1}
 \beta^{pt}= \{\beta^{pt}_k\}_{k=1}^{L}=
f_{h}(\mathbf{e}^p,\mathbf{e}^t;\Theta_{h})  
\end{equation}

where $k$ denotes layer number of transformer with $L$ layers, $\mathbf{e}^p$ is frozen and only current task embedding $\mathbf{e}^t$ is learnt along with \textit{MLP} and stored at the end of each task. These stored embeddings are used as input to \textit{MLP} to generate attention weights while learning new tasks. 



\textit{Linked Adapters} transfer the knowledge learnt by previous tasks through their adapters  to the current task, so that information from those tasks can be forwarded to the current task. This lateral connection is applied at every layer of the transformer network, and the intention of having weighted attention to the previous tasks is to ensure that only useful information is transferred to the current task. For current task \textit{t}, weighted lateral connections from previous tasks to current task at $k^{th}$ layer of transformer using \textit{Linked Adapters} can be defined as:

\begin{equation}\label{eq:3}
{\tilde{h}}^{t}_{k}= \sum_{p=1}^{t-1}  \beta^{pt}_{k} U^{p}_{k}(D^{p}_{k}( \bar{h}^{t}_{k}))+ \beta^{tt}_{k} U^{t}_{k}(D^{t}_{k}( \bar{h}^{t}_{k}).
\end{equation}

 % These attention weights are used to control information flow between lateral to subsequent tasks.
Here, $ \bar{h}^{t}_{k}$ is hidden state input to the adapter,  $\beta^{pt}_{k}$ are the corresponding attention weights computed with respect to current task $t$ that determine how much information to keep from previous task $p$, $ {\tilde{h}}^{t}_{k}$ is weighted attention computed over previous tasks. 

Let $h^{t}_{k-1}$ be the hidden representation output of $(k-1)^{th}$ transformer layer and input to $(k)^{th}$. Series of operations performed on $k^{th}$ layer of transformer can be defined as 
\begin{align*}
    &h_k^{'t} = {h}^{t}_{k-1} + \text{MHSA}(\text{Norm}({h}^{t}_{k-1})) \\
    &\bar{h}_k^{t}= \text{Norm}(h_k^{'t}))\\
    &\tilde{h}_k^{t} = \sum_{p=1}^{t-1} \beta_k^{pt} U_k^p(D_k^p(\bar{h}_k^{t})) + \beta_k^{tt} U_k^t(D_k^t(\bar{h}_k^{t})) \\
    &\hat{h}_k^{t} = \bar{h}_k^{t} + \tilde{h}_k^{t} \\
    &h^{t}_{k} = \bar{h}_k^{t} + \text{FFN}(\hat{h}_k^{t})
\end{align*}
where Norm, MHSA, FFN are the layer normalisation, Multi-Headed Self Attention, Feed Forward layers of $k^{th}$ layer of transformer respectively.




With the weighted lateral connections, knowledge from previous tasks can be forwarded to current learning task $t$. Learning a new task $t\in\mathcal{T}$ using \textit{Linked Adapters} can be defined as:
 \begin{align*}
    \max_{\Phi^{t},\mathbf{e}^t,\Theta_h,\Psi^t} \sum_{i=1}^{N^t} \log \mathcal{P}(y^t_i | x^t_i, \Theta^{\dagger},\Theta_{h},\mathbf{e}^t,\Phi^t, \Psi^t)
\end{align*}



% To mitigate the challenge of forgetting while updating the weights of the \textit{MLP} to generate attention weights across all tasks, the regularization technique online-EWC\cite{onlineewc} is employed. This strategy ensures that the \textit{MLP} can dynamically adapt to the current task without compromising the knowledge gained from previous tasks. The total loss to be optimized during the learning of the current task t is given by:

While attempting to learn on a new task, \textit{MLP} may overfit to the current task, which could cause it to lose the knowledge gained from previous tasks. To address this, we aim to regularize the \textit{MLP} parameters so that the MLP should be able to generate attention weights with respect to the previous tasks as well. The regularization over the \textit{MLP} parameters retain the values of the important \textit{MLP} parameters associated with the previous task learning stages similar to an Online-EWC~\cite{onlineewc}.  While learning the current task, the objective is to optimize the total loss which includes the task specific loss and the regularization term, and is defined as
\begin{equation}\label{eq:4}
\begin{split}
%\hspace{-0.09in}
\argmin_{\Theta_{h},\Phi^t,\Psi^t,\mathbf{e}^t} \mathcal{L}_{total} & =  \mathcal{L}_{task}(X^{t},Y^{t},\Theta_{h},\Theta^\dagger,\mathbf{e}^{t},\Phi^t,{\Psi^t}) \\ 
 & +{  {\lambda} \sum_{j}
 FI_{j}^{t-1}{(\Theta_{h,j}^{*} -\Theta_{h,j})^2 }} 
\end{split}
\end{equation}
where the first term
\(\mathcal{L}_{task}\) is task specific loss and the second term helps to regularise the \textit{MLP} weights to avoid forgetting, and $\lambda$ is the regularisation constant.  $\Theta_{h}^ {*}$ are \textit{MLP} weights after learning previous task and $\Theta_{h}$ are the \textit{MLP} weights that we are learning on the current task $t$.  $FI$ indicates fisher information matrix that computes the importance of weights $\Theta_{h}^ {*}$ in  \textit{MLP},  and the index $j$ iterates over all the \textit{MLP}  parameters. 


\begin{algorithm}
  \caption{Linked Adapters}
  \label{alg:example}
    \small
   \textbf{Require}: pre-trained model $\Theta,\mathcal{T}=\{\mathcal{T}^{1},\mathcal{T}^{2},\ldots,\mathcal{T}^{m}\} $ \\
   \textbf{During Training}:\\ 
  \hspace{0.3cm} Freeze $\Theta^{\dagger}$\\
  \hspace{0.3cm} Initialise MLP $\Theta_{h}$\\
  
  \hspace{0.3cm} \For{$t \leftarrow 1$ \KwTo $m$}{
     A new task $\mathcal{T}^t$ arrives\\
     Initialise adapter $\Phi^{t}$, embeddings $\mathbf{e}^t$, head $\Psi^{t}$;\\
     Generate forward attention weights $\beta^{pt}$ using \ref{eq:1}\\
     Add attention based forward connections
     \vspace{-0.35\baselineskip}
     \begin{algorithmic}
        \footnotesize
        \begin{align*}
        {\tilde{h}}^{t}_{k}= \sum_{p=1}^{t-1}  \beta^{pt}_{k} U^{p}_{k}(D^{p}_{k}( {\bar{h}}^{t}_{k}))+ \beta^{tt}_{k} U^{t}_{k}(D^{t}_{k}( {\bar{h}}^{t}_{k})
        \end{align*}
    \end{algorithmic}
    \vspace{-0.5\baselineskip}
 \\
     Optimise the model using $\mathcal{L}_{total}$ in \ref{eq:4} \\
     \textbf{After training task $t$}:\\
      \hspace{0.3cm} store $\Theta_{h}^*=\Theta_{h}^t$\\
      \hspace{0.3cm} Computer Fisher information matrix $FI$\\
      \hspace{0.3cm} Store and freeze $\Phi^{t}, e^{t}, \Psi^t$,  $\Theta_{h}^*$, $FI^t$   \\
     }
     
    \hspace{0.3cm}  
     
\textbf{During Testing}:  \\
% using   $\Theta_p^f,\Theta_h^f$,$e^{(f,{\scriptscriptstyle\leq} t)}$ 
\hspace{0.3cm}For a given input $x^t_i$ from some task t,\\
\hspace{0.3cm}Generate $\beta^{pt}$ and $\beta^{ts}$ using \ref{eq:5}\\ 
\hspace{0.3cm}Predict output $y^t_i$ considering both forward \\
\hspace{0.3cm} and backward connections  \\

\vspace{-1\baselineskip}
\begin{algorithmic}
        \scriptsize
        \begin{align*}
       {\tilde{h}}^{t}_k=&\sum_{p=1}^{t-1}\beta^{pt}_{k} U^{p}_{k}(D^{p}_{k}( \bar{h}^{t}_{k}))
        +\beta^{tt}_{k} U^{t}_{k}(D^{t}_{k}( \bar{h}^{t}_{k})+\\&\sum_{s=t+1}^{m}\beta^{ts}_{k} U^{s}_{k}(D^{s}_{k}( \bar{h}^{t}_{k}))
        \end{align*}
    \end{algorithmic}
    \vspace{-0.5\baselineskip}

\end{algorithm}




During regularising the weights of \textit{MLP},  \textit{Fisher Information Matrix (FI)} plays an important role by providing importance associated with them. This information is leveraged during the learning of the current task $t$ to ensure that important weights from previous tasks are constrained, thus preventing the risk of forgetting knowledge acquired over previous tasks. Before attempting to learn a new task $t$, importance assigned to weights of \textit{MLP} with respect to previous task $t-1$ $i.e.,$ $FI^{t-1}$ can be computed as
\begin{small}
\begin{align*}
   & FI^{t-1} =\\&\frac{1}{N^{t-1}} \sum_{j=1}^{N^{t-1}} \biggl [ \nabla_{\Theta_{h}^{*}} L_{task}(X^{t-1},Y^{t-1},\Theta_{h}^{*},\Theta^\dagger,\mathbf{e}^{t-1},\Phi^{t-1},{\Psi^{t-1}}) \nonumber \\ &\times  \nabla_{\Theta_{h}^{*}} L_{task}(X^{t-1},Y^{t-1},\Theta_{h}^{*},\Theta^\dagger,\mathbf{e}^{t-1},\Phi^{t-1},{\Psi^{t-1}})^T \biggl ]
\end{align*}
\end{small}
Here, $N^{t-1}$ represents the number of samples from task $t-1$ used for computing the \textit{FI}. We note that the derivatives are computed with respect to the \textit{MLP} parameters to assess the importance of those parameters.



\subsection{Linked Adapter Inference}
During training time, we restricted ourselves in considering only forward connection due to the CL setting.
We can also transfer knowledge acquired from subsequent tasks to the initial tasks that may not have received sufficient information. During the testing phase for the current task $t$, the model effectively employs lateral connections from both previous and subsequent tasks for knowledge transfer in the backward direction as in Figure~\ref{fig:architecture}.b. However, a challenge arises when generating attention weights for these lateral connections from subsequent tasks, as the degree of information flow from these tasks cannot be learned during the training phase. We address this challenge using a \textit{MLP} learnt during the training phase. \textit{MLP} facilitate the generation of attention weights for lateral connections from subsequent tasks to the current task without requiring any extra training. To achieve this, the \textit{MLP} takes task-specific embeddings of subsequent tasks as input, which are learned during the training phase, along with the current task embeddings and generate attention weights. 



During testing $t^{th}$ intermediate task after training on all $\mathcal{T}$ tasks, \textit{MLP} can generate forward attention weights $\beta^{pt}$ from the previous task \textit{p} to task \textit{t}  and  also backward attention weights  $\beta^{ts}$ from subsequent task \textit{s}  to task \textit{t}  can be defined as 

\begin{equation}\label{eq:5}
\begin{aligned}
 & \beta^{pt}= \{\beta^{pt}_k\}_{k=1}^{L}=
f_h(\mathbf{e}^p,\mathbf{e}^t;\Theta_{h}) \\ &
\beta^{ts} = \{\beta^{ts}_k\}_{k=1}^{L} = f_h(\mathbf{e}^t, \mathbf{e}^s; \Theta_{h})
\end{aligned}
\end{equation}
 For task $t$, weighted lateral connections using Linked Adapters from both previous and subsequent tasks at $k^{th}$ layer using \textit{MLP} generated attention weights can be defined as:
\begin{equation}\label{eq:7}
\footnotesize
{\tilde{h}}^{t}_k=\sum_{p=1}^{t-1}\beta^{pt}_{k} U^{p}_{k}(D^{p}_{k}( \bar{h}^{t}_{k}))
        +\beta^{tt}_{k} U^{t}_{k}(D^{t}_{k}( \bar{h}^{t}_{k})+\sum_{s=t+1}^{m}\beta^{ts}_{k} U^{s}_{k}(D^{s}_{k}( \bar{h}^{t}_{k}))
\end{equation}
Using these backward connections, subsequent tasks able to transfer knowledge to lateral tasks in backward directioncan see in Algorithm \ref{alg:example}.

By using \textit{Linked Adapters}, the pre-trained model can be fine-tuned for multiple tasks without requiring significant additional training or computational resources. This approach is especially useful when dealing with tasks that share some underlying structure or knowledge, as it allows the model to leverage this shared information to improve performance on multiple tasks. Specifically,  our \textit{Linked Adapters} is  compatible with all transformer-based architectures.


\section{ Experiments}
We performed extensive experiments on various image classification benchmarks to show
the effectiveness of our approach.  We consider two variants of our proposed approach to conduct experiments. 
\begin{itemize} [noitemsep]
\item \textit{AdaLink-Bidirectional} : the proposed  \textit{Linked Adapters} which allow knowledge transfer from previous and subsequent tasks. It considers weighted lateral connections from previous and later tasks at the test time. 
\item \textit{AdaLink-forward} : the variant of the  \textit{Linked Adapters} which allow knowledge transfer only  from previous tasks. This model considers weighted lateral connections only from previous tasks to the current tasks at the test time. 
\end{itemize}
We present our results on popular image classification data sets, \textit{CIFAR-10}~\cite{cifar100}, \textit{CIFAR100}~\cite{cifar100} and \textit{CUB200} ~\cite{cub200} datasets.


\textbf{Experimental Setup}: We aimed to perform experiments in task incremental setup where task identity is provided both during training and test time. For our experiments, we used pre-trained Vision Transformer ($ViT\_B\_16$) as the base network. 

\textbf{Baselines}:The approach we proposed is being evaluated against several established baseline methodologies in the field of continual learning. The benchmarks we are comparing our approach with are as follows:
\begin{itemize} [noitemsep]
\item \textit{Finetuning }: In this setting, model parameters adapt to new task without any constraints.

\item \textit{EWC} \cite{kirkpatrick2017overcoming}: It imposes constraints on the model parameters that are important to the old tasks while also allowing other parameters to adapt to new tasks
\item \textit{Experience Replay (ER)} \cite{experience}: This approach involves storing samples from previous tasks and replaying them while learning new tasks.

\item \textit{Adapters} \cite{houlsby2019parameter} : This setting learns separate and independent adapter module for each task. It clearly has no knowledge transfer or forgetting.
\end{itemize}


\textbf{Evaluation Metrics}: We use the standard evaluation metric of computing the averaged accuracy across all the tasks after training sequentially on the tasks.  To validate the effectiveness of \textit{AdaLink} in enabling knowledge transfer over sequence of tasks, we compute a \textit{knowledge Transfer(KT)} metric. For \textit{AdaLink}, the average knowledge transfer across all the tasks can be computed as $KT=\frac{1}{m}\sum_{i=1}^{m} {acc}_{link,i} - {acc}_{a,i} $ where ${acc}_{link,i}$ is accuracy of $i^{th}$  task using \textit{AdaLink}, ${acc}_{a,i}$ is accuracy of  $i^{th}$  task trained using separate and independent adapter approach.



\textbf{Datasets}:The proposed approach was evaluated on the \textit{Split-CIFAR10} dataset containing 10 classes, splitted into 5 tasks, each comprising 2 disjoint classes. Evaluation was also conducted on the \textit{Split-CIFAR100} dataset, splitting into 5 tasks, 10 tasks, and 20 tasks to demonstrate the approach's adaptability to various task sequences. Furthermore, the approach was evaluated on \textit{CUB200} dataset, containing images of 200 bird subcategories, with evaluations performed on splits of 5 and 10 tasks. 

In the following sections, we refer \textit{Linked Adapters} having only forward connection as \textit{AdaLink-Forward} and   \textit{Linked Adapters} with both forward and backward connections as \textit{AdaLink-Bidirectional}. 


\begin{table*}
\caption{Comparison of average test accuracy ($\%$) across various splits of \textit{Cifar-10, Cifar-100 and CUB-200} datasets (computed over 5 random seed initializations).
}

\resizebox{\textwidth}{!}{%
\begin{tabular}{|p{3.3cm}|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Split-Cifar-10} &
  \multicolumn{3}{c|}{Split-Cifar-100} &
  \multicolumn{2}{c|}{Split-CUB-200} \\ \hline
 &
  5 tasks &
  5 tasks &
  10 tasks &
  20 tasks &
  5 tasks &
  10 tasks  \\ \hline
\textit{Finetuning}    & 97.32 \scriptsize$\pm$ 1.54 & 92.64  \scriptsize$\pm$ 0.57 &94.44  \scriptsize$\pm$ 0.49 &  96.25  \scriptsize$\pm$ 0.59 & 77.93  \scriptsize$\pm$  0.41 &  77.64  \scriptsize$\pm$ 0.68  \\
\textit{EWC}           &  98.13  \scriptsize$\pm$ 0.56&  92.89  \scriptsize$\pm$ 0.40 &  95.03  \scriptsize$\pm$ 0.45 &  96.42  \scriptsize$\pm$ 0.96 & 78.02  \scriptsize$\pm$ 0.95 &  78.07  \scriptsize$\pm$ 0.58  \\
\textit{ER}            &  98.03  \scriptsize$\pm$ 0.39 & 93.27  \scriptsize$\pm$ 0.42 & 95.69  \scriptsize$\pm$ 0.50 & 97.19  \scriptsize$\pm$ 0.31 & 78.94  \scriptsize$\pm$ 0.94 & 78.31  \scriptsize$\pm$ 0.83 \\
\textit{Adapters}      & 99.34  \scriptsize$\pm$ 0.07 & 94.41  \scriptsize$\pm$ 0.10 & 96.57  \scriptsize$\pm$ 0.24 & 97.99  \scriptsize$\pm$ 0.14 &80.81  \scriptsize$\pm$ 1.22 & 80.51  \scriptsize$\pm$ 1.28 \\
\hline
\textit{AdaLink-Forward}      & 99.51  \scriptsize$\pm$ 0.03 & 95.66  \scriptsize$\pm$ 0.18 &97.39  \scriptsize$\pm$ 0.16 & 98.50  \scriptsize$\pm$ 0.14&  82.46  \scriptsize$\pm$ 1.21 & 80.94  \scriptsize$\pm$ 1.12 \\

 \textit{AdaLink-Bidirectional}   & \textbf{99.61  \scriptsize$\pm$ 0.02} & \textbf{95.96  \scriptsize$\pm$ 0.31} & \textbf{97.73  \scriptsize$\pm$ 0.21}  & \textbf{98.57  \scriptsize$\pm$ 0.18} & \textbf{82.76  \scriptsize$\pm$ 1.03} & \textbf{81.59  \scriptsize$\pm$ 0.83}  \\ \hline
\end{tabular}%
}
\label{table:1}
\end{table*}


\begin{table*}
\caption{ Average Knowledge Transfer (\%) across the tasks in AdaLink-Forward and AdaLink-Bidirectional in comparison to standalone adapters, where it has no knowledge transfer. 
}
\centering
% \small
% \resizebox{\textwidth}{!}{%
\begin{tabular}{|p{3.3cm}|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Split-Cifar-10} &
  \multicolumn{3}{c|}{Split-Cifar-100} &
  \multicolumn{2}{c|}{Split-CUB-200} \\ \hline
 &
  5 tasks &
  5 tasks &
  10 tasks &
  20 tasks &
  5 tasks &
  10 tasks  \\ \hline
\textit{AdaLink-Forward}      &0.17 &1.25&0.82&0.51& 1.65&0.43\\
\hline
 \textit{AdaLink-Bidirectional}    &0.27&1.55&1.16&0.58&1.95&1.08\\ \hline
\end{tabular}%
%}
\label{table:2}
\end{table*}




\section{ Results}

We compare the performance of the proposed approach with baselines on the image classification data sets, \textit{CIFAR-10}, \textit{CIFAR100} and \textit{CUB200} datasets in Table~\ref{table:1}. 

\subsection{Split-CIFAR10}
 Our proposed approach \textit{AdaLink-Forward} outperformed all the baseline specifically standalone Adapters approach  by enabling knowledge transfer of \textit{0.17\%} even on almost saturated \textit{Split-CIFAR10} results can be seen in Table~\ref{table:2}. Additionally, \textit{AdaLink-Bidirectional} able to transfer knowledge from both the directions by leveraging lateral connections with \textit{MLP} based weighted attention improved the performance by \textit{0.27\%} compared to standalone Adapters.
 



\subsection{Split-CIFAR100}

On the Split-CIFAR100 dataset, the \textit{AdaLink-Forward} approach consistently outperformed all baseline models across the three splits. Notably, when applied to the Split-CIFAR100 dataset with 5 splits, \textit{AdaLink-Forward} demonstrated a remarkable 1.25\% improvement in knowledge transfer can be seen in Table~\ref{table:2}, a substantial enhancement compared to standalone adapters that do not facilitate knowledge transfer. The efficacy of \textit{AdaLink-Forward} in transferring knowledge from prior tasks using lateral connections with \textit{MLP} based weighted attention to regulate the flow of information is evident in Figure~\ref{fig:sub1}. During testing, our proposed approach with \textit{AdaLink-Bidirectional} adeptly harnesses knowledge from both previous and subsequent tasks. In Figure~\ref{fig:sub1}, \textit{AdaLink-Bidirectional}  showcases its ability to transfer knowledge to initial tasks from subsequent tasks, resulting in performance improvements compared to \textit{AdaLink-Forward}, which solely relies on connections from previous tasks. By employing \textit{MLP} learnt during training, \textit{AdaLink-Bidirectional} able to improve knowledge transfer by 1.55\% compared to Adapters. This demonstrates the effectiveness of \textit{MLP} based weighted attention in enabling knowledge transfer from subsequent tasks, affirming its role in enhancing performance without the need for additional training. Similarly, on Split-CIFAR100 with 10 splits, \textit{AdaLink-Forward} exhibited an improvement in performance by 0.82\% can see in Table~\ref{table:2}. Furthermore, \textit{AdaLink-Bidirectional}, which includes both forward and backward connections, resulted better performance of 1.16\% is evident in  Figure~\ref{fig:sub2}. We extended our experiments to longer task sequences by splitting Split-CIFAR100 into 20 tasks to demonstrate the capability of our proposed method to transfer knowledge across longer sequences. \textit{AdaLink-Forward} showcased an improved performance by 0.51\%, and \textit{AdaLink-Bidirectional} has shown  0.58\% knolwedge transfer.


\begin{figure*}
    \centering
    
    \begin{subfigure}{0.49\textwidth}
        \includegraphics[width=\linewidth]{sec/a.png}
        \caption{}
        \label{fig:sub1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \includegraphics[width=\linewidth]{sec/b.png}
        \caption{}
        \label{fig:sub2}
    \end{subfigure}
    
    \vspace{1em}
    
    \begin{subfigure}{0.49\textwidth}
        \includegraphics[width=\linewidth]{sec/c.png}
        \caption{}
        \label{fig:sub3}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \includegraphics[width=\linewidth]{sec/d.png}
        \caption{}
        \label{fig:sub4}
    \end{subfigure}

    \caption{ Comparison between baselines and \textit{AdaLink} over average test accuracy of individual tasks. In the above figure, on X-axis tasks numbers are mentioned and on Y-axis, average test accuracy of individual tasks are presented }
    \label{fig:overall}
\end{figure*}



\subsection{Split-CUB200}

On the Split-CUB200 dataset with 5 splits, \textit{AdaLink-Forward} demonstrated its effectiveness by outperforming all baseline models, showcasing a substantial improvement of 1.65\% over standalone adapters can see in Table~\ref{table:2}. This notable knowledge transfer across tasks showcases the effectiveness of weighted attention based \textit{AdaLink-Forward} in facilitating knowledge from previous tasks. Furthermore, \textit{AdaLink-bidirectional}, considering both forward and backward connections, achieved an 1.95\% knowledge transfer over adapters, emphasizing the effectiveness of knowledge transfer across the tasks can be seen in Figure~\ref{fig:sub3}. Similarly, on 10 splits, \textit{AdaLink-Forward} exhibited a knowledge transfer of 0.43\% over standalone adapters. \textit{AdaLink-Bidirectional} continued to demonstrate its effectiveness by achieving a 1.08\% enhancement over Adapters can be seen in Figure~\ref{fig:sub4}.

In the experiments detailed in Table \ref{table:1}, approaches that employ adapters have a parameter growth of approximately 2\% for every task compared to the parameters present in the $ViT\_B\_16$. While, \textit{MLP} introduced for generating attention weights only adds 0.000034\% additional parameters across all tasks compared to the $ViT\_B_\_16$ which is nearly negligible.

These results effectively demonstrate the efficiency of the proposed approaches. \textit{AdaLink-Forward} successfully transfers knowledge from previous tasks, as indicated by the results. The incorporation of MLP-based weighted attention enables the learning of the degree of information flow from previous tasks to the current task. Furthermore, during testing, \textit{AdaLink-Bidirectional}, equipped with MLP-based weighted attention, efficiently acquires knowledge from both directions without requiring additional training.











\section{Conclusion}

This paper presents \textit{Linked Adapters}- a novel approach for continual learning that addresses knowledge transfer in PLMs. Our proposed approach, \textit{MLP} based \textit{Linked Adapters} establishes systematic lateral connections between task adapters to enable the knowledge transfer. The incorporation of attention weights, guided by a \textit{MLP}, addresses the challenge of determining information flow between tasks. During training, the \textit{MLP} learns to generate attention weights, enabling the current task model to selectively gain knowledge from preceding tasks. During testing, the trained \textit{MLP} proves instrumental in predicting attention weights for subsequent tasks, facilitating knowledge transfer without additional training. Experiments demonstrated the effectivenss of \textit{Linked Adapters} as a flexible and effective approach for continual learning with pre-trained transformer models.


==> sec/3_finalcopy.tex <==
\cleardoublepage
\thispagestyle{empty}
\begin{figure*}
    \centering
    
    \begin{subfigure}{0.49\textwidth}
        \includegraphics[width=\linewidth]{sec/a_std.png}
        \caption{}
        \label{fig:sub1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \includegraphics[width=\linewidth]{sec/b_std.png}
        \caption{}
        \label{fig:sub2}
    \end{subfigure}
    
    \vspace{1em}
    
    \begin{subfigure}{0.49\textwidth}
        \includegraphics[width=\linewidth]{sec/c_std.png}
        \caption{}
        \label{fig:sub3}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \includegraphics[width=\linewidth]{sec/d_std.png}
        \caption{}
        \label{fig:sub4}
    \end{subfigure}

    \caption{ Comparison between baselines and \textit{AdaLink} over average test accuracy of individual tasks. In the above figure, on X-axis tasks numbers are mentioned and on Y-axis, average test accuracy of individual tasks are presented (computed over 5 random seed initialisations) }
    \label{fig:overall_std}
\end{figure*}

\section{Supplementary}


In our experiments on the CUB-200-5splits dataset, we evaluated the knowledge transfer capabilities of our proposed models, Adalink-forward and Adalink-bidirectional, under varying task orders. Unlike traditional experiments where tasks are presented in a fixed order, we intentionally introduced randomized task sequences to demonstrate effectiveness of proposed approaches in knowledge transfer across tasks irrespective of task order.
Throughout the experiments, both AdaLink-forward and AdaLink-bidirectional consistently demonstrated robust knowledge transfer, showcasing their resilience to changes in task order. AdaLink-forward effectively utilized lateral connections to transfer knowledge from previous tasks to the current one. The forward attention weights, generated by the MLP, seamlessly adjusted to different task orders, ensuring the selective retention of information across the entire task sequence. Notably, AdaLink-bidirectional outperformed both standalone adapters and AdaLink-forward in all the task orders.






\subsection{Backward Transfer}
 To validate the effectiveness of \textit{AdaLink-Bidirectional} in enabling Backward Transfer over sequence of tasks, we compute a \textit{Backward Transfer(BT)} metric. The average backward transfer across all the tasks can be computed as $BT=\frac{1}{m}\sum_{i=1}^{m} {acc}_{end,i} - {acc}_{during,i}$. Here, ${acc}_{end,i}$ represents the accuracy achieved on the $i^{th}$ task when using \textit{AdaLink-Bidirectional} after training on all tasks, and ${acc}_{during,i}$ denotes the accuracy on the $i^{th}$ task when trained and tested after the $i^{th}$ task in the sequential order.


 The reported Average backward transfer of 0.35\% on Cub 200 5-splits and 0.38\% on Cub 200 with 10 splits showcase the capability of the proposed \textit{AdaLink-Bidirectional} approach in transferring knowledge in the backward direction, as detailed in Table \ref{tab:back}. The individual task accuracies of \textit{AdaLink} during Training are computed by evaluating accuracy for each task after its dedicated training phase. Furthermore, \textit{AdaLink-Bidirectional}, as illustrated in Figure \ref{fig:back}, emphasizes its ability to enhance knowledge transfer in backward directions.



\begin{table}
    \centering
    \caption{Average backward transfer(BT) Values for Cub Datasets}
    \begin{tabular}{|c|c|}
        \hline
        \textbf{Cub200 } & \textbf{BT(\%)} \\
        \hline
        5 Splits & 0.35\\
        \hline
        10 Splits & 0.38 \\
        \hline
    \end{tabular}
    \label{tab:back}
\end{table}
 

 \begin{figure*}
    \centering
    
    \begin{subfigure}{0.49\textwidth}
        \includegraphics[width=\linewidth]{sec/back-5.png}
        \caption{}
        \label{fig:sub1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \includegraphics[width=\linewidth]{sec/back-10.png}
        \caption{}
        \label{fig:sub2}
    \end{subfigure}
      \caption{Comparing indvidiual task accuracy(\%): AdaLink during Training vs. AdaLink Bidirectional. Here, AdaLink during Training refers computing accuracy for task after its dedicated training phase. In the above figure, on X-axis tasks numbers are mentioned and on Y-axis, average test accuracy of individual tasks are presented }
    \label{fig:back}
\end{figure*}
